MIMO Is All You Need : A Strong Multi-In-Multi-Out Baseline for Video Prediction

The mainstream of the existing approaches for video prediction builds up their models based on a Single-In-Single-Out (SISO) architecture, which takes the current frame as input to predict the next frame in a recursive manner. This way often leads to severe performance degradation when they try to extrapolate a longer period of future, thus limiting the practical use of the prediction model. Alternatively, a Multi-In-Multi-Out (MIMO) architecture that outputs all the future frames at one shot naturally breaks the recursive manner and therefore prevents error accumulation. However, only a few MIMO models for video prediction are proposed and they only achieve inferior performance due to the date. The real strength of the MIMO model in this area is not well noticed and is largely under-explored. Motivated by that, we conduct a comprehensive investigation in this paper to thoroughly exploit how far a simple MIMO architecture can go. Surprisingly, our empirical studies reveal that a simple MIMO model can outperform the state-of-the-art work with a large margin much more than expected, especially in dealing with longterm error accumulation. After exploring a number of ways and designs, we propose a new MIMO architecture based on extending the pure Transformer with local spatio-temporal blocks and a new multi-output decoder, namely MIMO-VP, to establish a new standard in video prediction. We evaluate our model in four highly competitive benchmarks (Moving MNIST, Human3.6M, Weather, KITTI). Extensive experiments show that our model wins 1st place on all the benchmarks with remarkable performance gains and surpasses the best SISO model in all aspects including efficiency, quantity, and quality. We believe our model can serve as a new baseline to facilitate the future research of video prediction tasks. The code will be released.

==> PaperBody/conclusion.tex <==
In this paper, we propose a Multiple-In-Multiple-Out (MIMO) strategy for video prediction, which generates the whole sequence of interest in parallel.
It overcomes the long-term dependencies and error accumulation problems inherently raised in the Single-In-Single-Out (SISO) strategy of existing RNNs.
The MIMO strategy can also improve prediction accuracy by maintaining the dependency among the future frames.
Based on this strategy, we present a MIMO Video Prediction model with convolutional Transformers (Predormer) for accurate prediction.
Predormer captures the long-term and short-term spatiotemporal relationships of sequences based on the convolutional structure and multi-head attention mechanism.
We conduct extensive ablation experiments to investigate the validity of the MIMO predictive strategy and model design.
Experimental results reveal that our Predormer achieves state-of-the-art performance on different kinds of datasets.
 
%Existing SISO methods for modeling spatiotemporal sequences can produce comparable results, but the ability to modeling more complicated dataset is still limited due to the  notorious long-term  dependencies  and  error  accumulation problem. 
%To address this issue, we propose a Multiple-In-Multiple-Out (MIMO) strategy  to infer the whole prediction sequence at once, and a new architecture called Predormer, which contains a 2D multi-head attention (2DMHA) to capture the long-term spatiotemporal dependencies and 3D Feed-Forward Network (3DFFN) to capture short-term correlations within sequences. Quantitative comparison results reveal that our proposed Predromer achieves state-of-the-art performance on different kinds of datasets.
 
%\noindent \textbf{Limitation.} Our MIMO strategy infers the whole sequence in parallel, which requires larger GPU memory than RNNs. 
%In addition, the self-attention operation is quadratically increased with the increased size of image sequences.
%Lastly, the MIMO strategy is lack of flexibility, which can not be used to predict future frames with variable output length.

%The proposed Predormer encodes the whole input sequences at once, which needs significantly large GPU memory.  Furthemore, the self-attention operation is quadratically increase with input length, which can be optimize in future works . Lastly, the MIMO strategy is not flexible, which can not be used to predict future frames with variational output length.

==> PaperBody/conclusion2.tex <==
In this paper, we propose a new MIMO architecture for video prediction, which overcomes the long-term dependencies and error accumulation problems inherently introduced in the Single-In-Single-Out (SISO) models. Extensive experiments have been conducted to verify our findings. Our model MIMO-VP achieves the top performance on all benchmarks and reveal the importance of MIMO for video prediction. We believe our model can serve as a new baseline in the video prediction area and rise the attention of the study for MIMO strategy in the future. 



==> PaperBody/experiment.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/attention.pdf}
	\caption{The attention maps of MIMO-VP, at $4$-th layer with the sum of 8 heads: (a) cross-attention map shows that the generated frames have high attention scores with the distant historical frames; (b) self-attention map indicates the dependency among the future frames;
	(c) an illustration of dependency between the predicted frame 51 and the other frames. 
	}
	\label{fig:attention}
\end{figure*}

We evaluated the proposed MIMO-VP on four video prediction datasets, Moving-MNIST dataset\cite{srivastava2015unsupervised}, Human 3.6M \cite{ionescu2013human3}  dataset, KITTI dataset and weather dataset. All the models were trained using the ADAM optimizer \cite{kingma2014adam}  and implemented in Pytorch. We first show the effect of MIMO strategy, which is detailed in  \cref{sec:Why MIMO beats SISO?}. Then, in  \cref{sec:Which MIMO?}, we carry out an ablation study on the Moving MNIST dataset to show the effectiveness of our design. Lastly, the quantitative results on each dataset is shown in  \cref{sec:IS MIMO beats SISO ?}.  

\subsection{Dataset Descriptions}
% We evaluate our MIMO-VP on four challenging benchmarks with one synthetic dataset and three real-world datasets. 

\noindent \textbf{Moving MNIST} \cite{srivastava2015unsupervised} is a standard synthetic dataset for video prediction.
It contains two handwritten digits that move along time at a fixed velocity and a random initial direction within a $64$$\times$$64$ size image. 
We generate the training set following the method in \cite{guen2020disentangling},
and adopt the widely used test set of 10,000 sequences provided by \cite{srivastava2015unsupervised} for evaluation. 

\noindent \textbf{Human3.6M} \cite{ionescu2013human3} dataset is a real-world human pose dataset comprising 17 kinds of human actions and 3.6 million poses.  
Human actions are stochastic, and different parts of the human body also have diverse transient variations, which brings great challenges to the prediction tasks.
In our experiments, all the RGB images are center-cropped to a resolution of 800$\times$800$\times$3 and then resized to 128$\times$128$\times$3.
We use subjects S1, S5, S6, S7 and S8 for training, and subjects S9, S11 for testing. 
We predict $4$ frames in the future conditioned on the $4$ observed frames.

\noindent \textbf{Weather} dataset is a real radar echo dataset for precipitation nowcasting, which is generated and processed from the local weather bureau.
Precipitation nowcasting is vital challenging because of the distortion, dissipation and accumulation of radar echoes.
The Weather dataset consists of $12,000$ consecutive radar sequences with each sequence of 20 frames, collected every 12 minutes.
In our experiments, the training set contains $9,600$ radar sequences with a resolution of 128$\times$128$\times$1, and the test set contains $2,400$ sequences.

\noindent \textbf{KITTI} dataset is one of the most popular datasets for autonomous driving and also a benchmark for computer vision algorithms. 
It is composed of hours of traffic scenarios recorded with a variety of sensor modalities, including high-resolution RGB images, gray-scale stereo cameras, and a 3D laser scanner. 
Due to the variability of camera position and street views, predicting on the KITTI dataset becomes extremely difficult challenge.
We predict $5$ frames in the future taking $5$ observed frames as input.

\begin{figure}
	\centering
	\begin{subfigure}[]{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/long-term.pdf}
		\caption{MSE w.r.t input length}
		\label{figure:long-term}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/error.pdf}
		\caption{Frame-wise MSE}
		\label{figure:error accumulation}
	\end{subfigure}
	\caption{(a) Comparison of MIMO-VP and PhyDNet by predicting 10 future frames conditioned on different length of input sequence; (b) Frame-wise MSE of MIMO-VP and PhyDNet on Moving MNIST dataset.}
\end{figure}




\begin{figure}
	\centering
	\begin{subfigure}[]{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/longterm-mae.pdf}
		\caption{MAE w.r.t Output length}
		\label{figure:long term prediction1}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/longterm-ssim.pdf}
		\caption{SSIM w.r.t Output length}
		\label{figure:long term prediction2}
	\end{subfigure}
	\caption{The mean MAE (a) and SSIM (b) by using 10 frames to  predict 10, 30, 50 and 90 frames.}
\end{figure}



\subsection{Evaluation Metrics}
To evaluate the performance of our MIMO-VP against previous state-of-the-art works in deterministic prediction domain, 
\ie LMC-Memory\cite{lee2021video}, 
MotionRNN \cite{wu2021motionrnn}, 
PhyDNet \cite{guen2020disentangling}, 
Conv-TT-LSTM \cite{su2020convolutional}, 
CrevNet \cite{yu2019crevnet}, 
MIM\cite{wang2019memory} and ConvLSTM \cite{xingjian2015convolutional}, 
several metrics are used in our experiment, 
including Mean Squared Error (MSE), 
Mean Absolute Error (MAE), 
the Structural Similarity (SSIM), 
LPIPS\cite{zhang2018unreasonable} and Peak Signal to Noise Ratio (PSNR). 
All these metrics are averaged for all predicted frames. 
Lower MSE, MAE, LPIPS, or higher SSIM, PSNR indicates better performance. 
In addition, for Weather dataset, we also take Critical Success Index (CSI) into account. 
The CSI score is a significant evaluation metric in precipitation nowcasting domain, which is calculated as:
\begin{equation}
CSI = \frac{hits}{hits+misses+false alarms}, 
\end{equation}
where \textit{hits}, \textit{misses} and \textit{falsealarms} denote the number of\textit{ true positive},\textit{ false positive} and \textit{false negative}, respectively. 
The higher the CSI score, the better the performance. 

% \subsection{Implementation Details}
% We use Adam \cite{kingma2014adam} with 0.0005 learning rate to train our model. ReduceLROnPlateau is adopted to reduce the learning rate with 0.5 decay factor when loss stop decreasing. For Moving MNIST dataset, we use 6 transformer blocks in the encoder and 10 transformer blocks in the decoder. While for other three datasets, we use both 6 blocks in the encoder and decoder modules. 
% The model channel is set to be $C=128$. 
% We use 8 heads in our 2DMHA module.
% The batch size is set to be 32 for Moving MNIST dataset and 8 for other datasets. 
% We implemented the model with PyTorch and conducted experiments on NVIDIA V100 GPUs.




\subsection{Why MIMO beats SISO?}
\label{sec:Why MIMO beats SISO?}
\subsubsection{\textbf{Less Error Accumulation}}
\Cref{figure:error accumulation} illustrates the frame-wise MSE results of MIMO-VP and PhyDNet, corresponding to the sample in \Cref{fig:mnist}, and lower curves denote higher prediction accuracy.
We observe that the frame wise mse of PhyDNet is increase obviously when compared with our MIMO-VP.
In \Cref{fig:mnist}, the predicted frames of PhyDNet and MotionRNN become distorted and blurry, and their prediction error largen over time,
while the predicted sequence of MIMO-VP still maintains high quality.
These comparison results prove that with the help of MIMO strategy, MIMO-VP can overcome the error accumulation.
\subsubsection{\textbf{Future Frame Dependency}}
We compare our MIMO-VP with its variant \textit{MIMO-VP\_independent}, a method that removes the self-attention module and replaces the 3DFFN with 2DFFN in the decoder module, to remove the dependency between future frames. 
Predictive results are shown in \Cref{Tab: dependncy of future},
from which we can see MIMO-VP achieves much better performance than \textit{MIMO-VP\_independent}.
In addition, the self-attention map in \Cref{fig:attention} (b) shows that each predicted frame has high attention scores with its neighboring frames, indicating their dependency.
This phenomenon verifies the benefit of MIMO-VP in preserving the dependency among the future frames for accurate prediction.



\subsubsection{\textbf{Long range dependency}} In this section, we will discuss the effectiveness of our MIMO-VP in long-term case from the point of variational input length and output length. \\
\noindent \textbf{Significance of 'MI'.}
To investigate how the MIMO-VP is capable of capturing the long-term relationships of sequence,
we conduct experiment on Moving mnist dataset by predicting 10 future frames conditioned on $50$ observed frames.
The cross-attention map in \Cref{fig:attention} (a) shows that the predicted frames have stronger attentions with the distant input frames (small index of frames),
which indicates that MIMO-VP can leverage the distant historical information of sequence based on the 2DMHA mechanism to facilitate the future frame generation.
For example, \Cref{fig:attention} (c) shows that the input frames 4, 5, 6, 7, 28, 29 and 45 are helpful for predicting frame 51.
We also investigate the influence of the length of the input sequence.
%Experiment results of predicting 10 future frames of MIMO-VP and PhyDNet on Moving MNIST dataset with different length of input sequences are shown \Cref{fig:long-term}.
Comparison results between MIMO-VP and PhyDNet of predicting 10 future frames on Moving MNIST with different input lengths are shown in \Cref{figure:long-term}.
It is observed that the MSE metric of MIMO-VP drops quickly with the input length increasing from 5 to 50.
PhyDNet improves significantly when the input length increases from 5 to 10,
while improves slightly from 10 to 50.
Precisely, the MSE of MIMO-VP and PhyDNet deceases by $64.3\%$ and $24.4\%$ respectively from 10 input frames to 50 input frames.
Those results demonstrate that our MIMO-VP has a stronger ability to capture the long-term sptiotemporal dependency of video sequences for accurate prediction,
while PhyDNet, an RNN-based method, suffers from the long-term dependency problem because of the limited capacity of memory.

\noindent \textbf{Significance of 'MO'.} To verify the effectiveness of the MIMO strategy on long-term prediction, we compare the results of predicting 10,30,50 and 90 frames on Moving MNIST dataset. 
In training phase, all the models are trained by using 10 frames to predict next 10 frames, while in testing phase, 10, 30, 50, and 90 frames are predicted in a recurrent manner. 
Experimental results are shown in Figure XXX, from which we can observe that our model achieve the state-of-the-art performance on all 4 long-term time scales. 
\begin{table}[t]
	\centering
	\tabcolsep9pt
	\caption{Comparison of MIMO-VP and its variant on Moving MNIST dataset.}
	%\small
	\begin{tabular}{l|ccc}
		\hline
		Method  & MSE $\downarrow$ & MAE $\downarrow$ & SSIM $\uparrow$ \\
		\hline 
		\hline
		MIMO-VP\_independent & 21.6 & 59.4 & 0.955 \\
		\textbf{MIMO-VP} & \textbf{17.7} & \textbf{51.6} & \textbf{0.964} \\
		\hline
	\end{tabular}
	\label{Tab: dependncy of future}
\end{table}


% \noindent \textbf{Influence of Error accumulation.}
% \Cref{fig:error accumulation} illustrates the frame-wise MSE results of Predomer and PhyDNet, corresponding to the sample in \Cref{fig:mnist}, and lower curves denote higher prediction accuracy.
% The curve of PhyDNet increase dramatically over time because PhyDNet suffers from the error accumulation problem, while the curve of MIMO-VP increase because the normal predictive error (related to the digit overlapping) increases over time..
% In \Cref{fig:mnist}, the predicted frames of PhyDNet and MotionRNN become distorted and blurry, and their prediction error largen over time,
% while the predicted sequence of MIMO-VP still maintains high quality.
% These comparison results prove that with the help of MIMO strategy, MIMO-VP can overcome the error accumulation. 

\subsubsection{\textbf{Efficient and Effective}}
From \Cref{Tab: Inference Time}, we can observe that our 'MO' methods runs much faster than 'SO' methods. According to \Cref{figure:long term prediction1}, \Cref{figure:long term prediction2}, we can see that MIMO-VP can achieve state-of-the-art performance with a comparable inference time, which can serve as a backbone for future research. 







\begin{table*}[h]
%\small
\centering
\tabcolsep3pt
\caption{Quantitative comparison of different models on Moving MNIST dataset.}
  \begin{tabular}{l|ccccc}
  \hline
    Method   & MSE & MAE $\downarrow$ & SSIM $\uparrow$\\
	\hline 
	\hline
		MAU \cite{chang2021mau} & 27.6 & 79.4 & 0.937   \\
	\hline	
	3D convolution \cite{yu2019crevnet} & 32.8 & 84.4 & -   \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 1005.3 & 4092.9 & 0.695\\
		ViT \cite{guen2020disentangling} & 50.2 & 126.5 & 0.887  \\
		Swin-transformer \cite{lee2021video}& 28.8 & 77.2 & 0.940  \\
		SimVP \cite{gao2022simvp}  & 23.8& 68.9 & 0.948 \\
		\textbf{MIMO-VP} & \textbf{17.7}  & \textbf{51.6} & \textbf{0.964}   \\
     \hline
	\end{tabular}
\label{Tab: MIMO_compare}
\end{table*}




\begin{table}[h]
%\small
\centering
\tabcolsep3pt
\caption{The inference time of different models on Moving MNIST dataset.}
  \begin{tabular}{l|ccccc}
  \hline
    Models   & PhyDNet & SimVP  & MotionRNN & MIMO-VP\\
	\hline 

	10-30 & 0.2274s & 0.0643s & 0.6299s & 0.1498s    \\

     \hline
	\end{tabular}
\label{Tab: Inference Time}
\end{table}




\subsection{Which MIMO?}
\label{sec:Which MIMO?}
\subsubsection{\textbf{MIMO vs Best SISO}}
The comparison of different MIMO methods and the best SISO method is shown in Table \ref{Tab: MIMO_compare}.  We first observe that all other MIMO methods can not achieve state-of-the-art performance when compared with the best SISO method--MAU \cite{chang2021mau}. We think the reason is that 3D convolution is a local operation and it neglects the global spatial dependency among features, while the vision transformer based models neglect the local spatial dependency due to the linear operation of features. However, we use 2DMHA and 3DFFN to track the global and local spatial-temporal dependency and finaly MIMO-VP achieves state-of-the-art performance. 
\subsubsection{\textbf{The effectiveness of our design}}
We perform an ablation study to analyse the respective contributions of the 2DMHA, the 3DFFN.
Accordingly, we compare MIMO-VP with its two variants:
(1) \textit{MIMO-VP w/o 2DMHA} is a fully 3D convolutional neural networks by removing 2DMHA modules, which is based on the MIMO strategy;
(2) \textit{MIMO-VP w/ 2DFFN}, a variant that replace the 3D convolutional in FFNs with 2D convolutional.
%(3) \textit{MIMO-VP w/ Recurrent} denotes a variant of MIMO-VP that adopts the predictive strategy similar to vanilla Transformer.
%It passes the shifted target sequence into the decoder, which infers one next frame using the predicted frames, in a recursive manner.
Quantitative results on Moving mnist and KITTI datasets are shown in \Cref{Tab: ablation}.
We can see that \textit{MIMO-VP w/o 2DMHA} shows much performance degradation in comparison with MIMO-VP,
with an increase of $15.1$ and $32.8$ in terms of MSE and MAE respectively on the Moving MNIST for example.
This phenomenon indicates that 2DMHA mechanism, which is able to capture the global long-term spatiotemporal relationships of sequences, makes an important contribution to the accurate video prediction.
The results of \textit{MIMO-VPw w/ 2DFFN} also show inferior to those of MIMO-VP, which verifies that the short-term variations of sequence are helpful for prediction.
%In summary, quantitative results in \Cref{Tab: ablation} fully prove that each component of MIMO-VP contribute to accurate prediction.

\begin{table*}[t]
	%\small
	\centering
	\tabcolsep8pt
	\caption{Quantitative comparison of different models on Moving MNIST dataset.}
	\begin{tabular}{l|ccc|ccc}
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c|}{10 - 10}& \multicolumn{3}{c}{10 - 30} \\
		\cline{2-7}
		& MSE  $\downarrow$ & MAE  $\downarrow$ & SSIM $\uparrow$& MSE  $\downarrow$ & MAE  $\downarrow$ & SSIM $\uparrow$\\
		\hline
		\hline
		ConvLSTM \cite{xingjian2015convolutional} & 103.3& 182.9 & 0.707 &-&-&-\\
		MIM \cite{wang2019memory} & 44.2 & 101.1 & 0.910 &-&-&- \\
		CrevNet \cite{yu2019crevnet} & 22.3 & - & 0.949 &-&-&- \\ \hdashline
		ConvTTLSTM \cite{su2020convolutional} & 56.0& 92.9& 0.913 & 105.7  & - & 0.840\\
		PhyDNet \cite{guen2020disentangling} & 24.2  & 70.3 & 0.947&58.7 & 144.1 & 0.852 \\
		LMC-Memory \cite{lee2021video} & 41.5  & - & 0.924 &73.2 & - & 0.879\\
		MotionRNN \cite{wu2021motionrnn} & 29.2  & 87.7& 0.933&64.2 & 156.1 & 0.844\\ 
		SimVP(\cite{gao2022simvp}) & 23.8 & 68.9 & 0.948 &-&-&- \\
		\hline
		\textbf{Predformer} & \textbf{17.7} & \textbf{51.6} & \textbf{0.964} & \textbf{31.6}& \textbf{79.1}& \textbf{0.934}\\
		\hline
	\end{tabular}
	\label{Tab: Moving MNIST}
\end{table*}

\begin{table}[t]
	%\small
	\centering
	\tabcolsep 1pt
	\caption{Quantitative comparison of different methods on Human3.6M dataset.}
	\begin{tabular}{l|ccc}
		\hline
		Method   & MAE/100 $\downarrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ \\
		\hline 
		\hline
		MIM \cite{yu2019crevnet} & 17.8& 0.790 & 20.57  \\
		PhyDNet \cite{guen2020disentangling} & 16.2 & 0.901 &-\\
		LMC-Memory \cite{lee2021video}  & 17.0 & 0.820 &21.05\\
		MotionRNN \cite{wu2021motionrnn}  & 14.8& 0.846 & 22.16   \\
		\textbf{Predformer}  & \textbf{10.4} & \textbf{0.941}  & \textbf{24.52} \\
		\hline
	\end{tabular}
	\label{Tab: human}
\end{table}

\subsubsection{\textbf{How to make the best design?}} 
We report the experimental results regarding the number of transformer blocks and the number of heads in 2DMHA in \Cref{Tab: model design}.
Generally, a deeper model with more layers of transformer will bring higher performance. 
For the trade-off of prediction accuracy and model efficiency,
we use '6-10' model on Moving MNIST, and '6-6' model on the other datasets.
We note that the results of multiple heads attention are better than single head in our experiment because multiple heads could effectively capture complicated long-term temporal cues for video prediction.
Therefore, we chose 8 heads in our MIMO-VP.

\noindent \textbf{Effectiveness of MIMO.}
To further verify the validity of our MIMO strategy, we compare MIMO-VP with several methods based on different predictive strategies and architectures.
Specially,
\textit{MIMO-VP\_r} denotes a variant of MIMO-VP that adopts the MISO predictive strategy similar to vanilla Transformer.
It passes the shifted target sequence into the decoder, and infers the next one frame using the last predicted frame, in a recursive manner.
HORST \cite{tai2021higher} is an encoder-only transformer-style architecture that adopts single-in-single-out recursive predictive strategy for video action recognition.
Experimental results are shown in \Cref{Tab: mimo},
from which we can observe that MIMO-VP obtains higher performance than \textit{MIMO-VP\_r},
especially on the Moving mnist dataset by predicting 10 future frames, with performance improves by $18.0\%$ and $14.0\%$ in MSE and MAE respectively.
Also MIMO-VP gains a significantly better performance improvement over PhyDNet and HORST on both datasets.
The reason may be that recursive single-out predictive strategy will trigger the error accumulation problem and overlook the stochastic dependency among the future frames.
These results fully prove the effectiveness of MIMO predictive strategy in video prediction.



% \subsection{Model Analysis}
\begin{table}[t]
	%\small
	\centering
	\tabcolsep0.8pt
	\caption{Comparison of MIMO-VP and its variant on Moving MNIST and KITTI datasets.}
	\begin{tabular}{l|cc|cc}
		\hline
		& \multicolumn{2}{c|}{Moving MNIST}  & \multicolumn{2}{c}{KITTI} \\
		\hline
		Method  & MSE $\downarrow$ & MAE $\downarrow$ & MAE/100 $\downarrow$ & SSIM $\uparrow$ \\
		\hline  
		\hline
		MIMO-VP\_independent & 21.6 & 59.4 & 41.5 & 0.695 \\
		MIMO-VP w/o 2DMHA & 32.8 & 84.4 & 44.6 & 0.663 \\
		MIMO-VP w/  2DFFN  & 21.2 & 59.2 & 42.3 & 0.687 \\
		%MIMO-VP w/ Recurrent & 22.8 & 62.8 & 42.1 & 0.690 \\
		\hline
		\textbf{MIMO-VP}  & \textbf{17.7} & \textbf{51.6} & \textbf{40.9}  & \textbf{0.703}  \\
		\hline
	\end{tabular}
	\label{Tab: ablation}
\end{table}

% The two key designs of our MIMO-VP is the MIMO strategy that infers the whole video sequence of interest at once and the transformer blocks to model the long-term and short-term spatiotemporal dependencies of sequences.
% We visualize and analyze their influence on Moving MNIST and KITTI datasets as below.
%In addition, we also report the experimental results regarding the model design in the supplementary material.




% \noindent \textbf{Influence of dependency of future.}
% We compare our MIMO-VP with its variant \textit{MIMO-VP\_independent}, a method that removes the self-attention module and replaces the 3DFFN with 2DFFN in the decoder module, to make the output frames independent.
% Predictive results are shown in \Cref{Tab: ablation},
% from which we can see MIMO-VP achieves much better performance than \textit{MIMO-VP\_independent}.
% In addition, the self-attention map in \cref{fig:attention} (b) shows that each predicted frame has high attention scores with its neighboring frames, indicating their dependency.
% This phenomenon verifies the benefit of MIMO-VP in preserving the dependency among the future frames for accurate prediction.

\begin{table*}[t]
	%\small
	\centering
	\tabcolsep3pt
	\caption{Quantitative comparison of different methods on Moving MNIST and KITTI datasets. In the third column, "R" and "T" denotes RNN and Transformer architecture respectively.}
	\begin{tabular}{l|c|c|cc|cc}
		\hline
		\multicolumn{3}{c|}{}& \multicolumn{2}{c|}{Moving MNIST}  & \multicolumn{2}{c}{KITTI} \\
		\hline
		Method  & Type & Network &MSE $\downarrow$ & MAE $\downarrow$ & MAE/100 $\downarrow$ & SSIM $\uparrow$ \\
		\hline 
		\hline
		PhyDNet \cite{guen2020disentangling} & SISO & R & 24.2 & 70.3 & 44.9 & 0.674 \\
		HORST \cite{tai2021higher} & SISO & T & 26.5 & 75.5 & 53.3 & 0.571 \\
		MIMO-VP\_r & MISO & T &22.8 & 62.8 & 42.1 & 0.690 \\
		\textbf{MIMO-VP} & MIMO & T & \textbf{17.7} & \textbf{51.6} & \textbf{40.9}  & \textbf{0.703}  \\
		\hline
	\end{tabular}
	\label{Tab: mimo}
\end{table*}

\begin{table}[t]
	%\small
	\centering
	\tabcolsep12pt
	\caption{Quantitative comparison of different designs of MIMO-VP on Moving MNIST dataset. Model 'a-b' denotes MIMO-VP with 'a' encoder blocks and 'b' decoder blocks.}
	\begin{tabular}{l|ccc}
		\hline
		Models   & MSE $\downarrow$ & MAE $ \uparrow$ & SSIM $\uparrow$ \\
		\hline 
		\hline
		4-8  & 19.3 & 55.4 & 0.960  \\
		\textbf{6-10} & 17.7 & 51.6 & 0.964 \\
		8-12 & 17.6 & 51.3 & 0.964  \\  
		\hline
		1 head & 19.1 & 55.0 & 0.960 \\
		4 heads & 18.0 & 52.4 & 0.963 \\
		\textbf{8 heads} & 17.7 & 51.6 & 0.964 \\
		16 heads & 18.1 & 52.7 & 0.963 \\
		\hline
	\end{tabular}
	\label{Tab: model design}
\end{table}


% \noindent \textbf{Ablation study.}
% We perform an ablation study to analyse the respective contributions of the 2DMHA, the 3DFFN and the MIMO strategy. 
% Accordingly, we compare MIMO-VP with its three variants:
% (1) \textit{MIMO-VP w/o 2DMHA} is a fully 3D convolutional neural networks by removing 2DMHA modules, which is based on the MIMO strategy;
% (2) \textit{MIMO-VP w/ 2DFFN}, a variant that replace the 3D convolutional in FFNs with 2D convolutional.
% %(3) \textit{MIMO-VP w/ Recurrent} denotes a variant of MIMO-VP that adopts the predictive strategy similar to vanilla Transformer.
% %It passes the shifted target sequence into the decoder, which infers one next frame using the predicted frames, in a recursive manner.
% Quantitative results on Moving mnist and KITTI datasets are shown in \Cref{Tab: ablation}.
% We can see that \textit{MIMO-VP w/o 2DMHA} shows much performance degradation in comparison with MIMO-VP,
% with an increase of $15.1$ and $32.8$ in terms of MSE and MAE respectively on the Moving MNIST for example.
% This phenomenon indicates that 2DMHA mechanism, which is able to capture the global long-term spatiotemporal relationships of sequences, makes an important contribution to the accurate video prediction.
% The results of \textit{MIMO-VPw w/ 2DFFN} also show inferior to those of MIMO-VP, which verifies that the short-term variations of sequence are helpful for prediction.
%In summary, quantitative results in \Cref{Tab: ablation} fully prove that each component of MIMO-VP contribute to accurate prediction.





\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{pictures/mnist.pdf}
	\caption{Prediction examples on Moving MNIST dataset. 
	}
	\label{fig:mnist}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{pictures/human.pdf}
	\caption{Prediction examples on Human3.6M dataset. 
	}
	\label{fig:human}
\end{figure}

% \noindent \textbf{Effectiveness of MIMO.}
% To further verify the validity of our MIMO strategy, we compare MIMO-VP with several methods based on different predictive strategies and architectures.
% Specially,
% \textit{MIMO-VP\_r} denotes a variant of MIMO-VP that adopts the MISO predictive strategy similar to vanilla Transformer.
% It passes the shifted target sequence into the decoder, and infers the next one frame using the last predicted frame, in a recursive manner.
% HORST \cite{tai2021higher} is an encoder-only transformer-style architecture that adopts single-in-single-out recursive predictive strategy for video action recognition.
% Experimental results are shown in \Cref{Tab: mimo},
% from which we can observe that MIMO-VP obtains higher performance than \textit{MIMO-VP\_r},
% especially on the Moving mnist dataset by predicting 10 future frames, with performance improves by $18.0\%$ and $14.0\%$ in MSE and MAE respectively.
% Also MIMO-VP gains a significantly better performance improvement over PhyDNet and HORST on both datasets.
% The reason may be that recursive single-out predictive strategy will trigger the error accumulation problem and overlook the stochastic dependency among the future frames.
% These results fully prove the effectiveness of MIMO predictive strategy in video prediction.




% \subsection{Comparison with State-of-the-arts}

% \noindent \textbf{Results on Moving MNIST.}
% Firstly, we evaluate the performance of our MIMO-VP with the state-of-the-art methods on 10-10 task, which means 10 frames are used to predict 10 future frames. 
% As shown in \Cref{Tab: Moving MNIST}, our model significantly outperforms all the other models.
% %gains a huge performance improvement and achieves the best performance. 
% In detail, compared with PhyDNet, our model improves $26.9\%$ and $26.6\%$in terms of MSE ans MAE respectively.  
% As shown in \Cref{fig:mnist}, at the beginning, the two digits stick together and then gradually keep away from each other.
% Current RNN-based models get blurry and wrong predictions in this case, and their prediction error largen over time.
% On the contrary, our model can predict precise and clear frames. 

% To further explore the performance of our MIMO-VP on long-term prediction, we conduct an experiment by predicting 30 future frames conditioned on 10 input frames. 
% As shown in \Cref{Tab: Moving MNIST}, our method far surpasses the others in predicting 30 frames in terms of the MSE metric. 
% Compared with PhyDNet, our MIMO-VP improves $46.2\%$ in MSE , which is much larger than $26.9\%$ in 10-10 prediction task. 
% From the comparison, we can conclude that our MIMO-VP captures the long-term spatiotemporal dependency both in the input frames and output frames. 
% Furthermore, our model has more advantages in predicting long-term sequences. 
%The visualization results of 10-30 task is shown in supplementary materials. 

\begin{table*}[h]
%\small
\centering
\tabcolsep3pt
\caption{Quantitative comparison of different models on KITTI dataset.}
  \begin{tabular}{l|cccc}
  \hline
    Method   & MAE/100 $\downarrow$ & SSIM $\uparrow$& LPIPS $\downarrow$ & PSNR $\uparrow$ \\
	\hline 
	\hline
	CrevNet \cite{yu2019crevnet} & 56.3 & 0.587  & 0.454  & 17.046  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 1005.3 & 4092.9 & 0.695\\
		PhyDNet \cite{guen2020disentangling}  & 44.9 & 0.674  & 0.403& 19.159 \\
		LMC-Memory \cite{lee2021video}  & 44.6 & 0.660  &  0.410  & 18.692\\
		MotionRNN \cite{wu2021motionrnn}  & 45.0 & 0.652  & 0.384& 18.931 \\
		\textbf{Predformer}  & \textbf{40.9} & \textbf{0.703} & \textbf{0.308}& \textbf{19.616}  \\
     \hline
	\end{tabular}
\label{Tab: kitti}
\end{table*}

\begin{table*}[h]
\centering
\caption{Quantitative comparison of different models on Weather dataset.}
\tabcolsep 8pt
  %\small
  \begin{tabular}{l|cccc}
  \hline
    Method  & MAE $\downarrow$ & SSIM $\uparrow$ & CSI-20 $\uparrow$ & CSI-30 $\uparrow$\\
	\hline 
	\hline
	MIM \cite{wang2019memory}  & 402.6 & 0.725& 0.402  & 0.164\\
		% 		CrevNet \cite{yu2019crevnet} & 962.4 & 0.786  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 51.0 & 223.0 & 0.847\\
		PhyDNet \cite{guen2020disentangling}  & 280.1 & 0.859 & 0.557 & 0.368 \\
		MotionRNN \cite{wu2021motionrnn}  & 336.9 & 0.809 & 0.519 & 0.290 \\
		\textbf{Predformer}  & \textbf{235.6} & \textbf{0.865} & \textbf{0.595} & \textbf{0.400}\\ 
     \hline
	\end{tabular}
\label{Tab: weather}
\end{table*}


% \noindent \textbf{Results on Human3.6M.}
% %Human action is one of the most difficult task in video prediction domain. 
% %From Table \ref{Tab: human}, we can see that our proposed MIMO-VP achieves the best performance compared with other methods. 
% %From Figure \ref{fig:human} we also can see that our model predicts comparable result with the state-of-the-art methods. 
% %However, we have to say the performance of all these models are not as perfect as we expect. 
% %Thesefore, how to model the non-rigid active of human body is a much challenging task, which is left for future work.
% \Cref{Tab: human} shows that MIMO-VP achieves the best performance on Human3.6M. 
% Compared with PhyDNet, MIMO-VP improves $35.8\%$ in MAE. 
% %In \Cref{fig:human}, the background is complicated and gives much more challenge for modeling. 
% %From the visualization results , we can see that our model still can product reasonable results while other models get quite blurry predictions.
% In \Cref{fig:human}, complicated background and human motion give much more challenge for predicting accurate and reasonable results. While our MIMO-VP can still product relatively precise future frames comparing with other models.
%Some approaches e.g.\cite{Ruben2018Longterm} uses human pose information as additional supervision.

% From Figure \ref{fig:human} we can see that in the result of LMC-Memory, obvious deformation appears on human legs. 
% In the result of MotionRNN and PhyDNet, the upper human body is unreasonably slim and obese comparing to groundtruth.
% While our model MIMO-VP can take into account the rationality of the overall human shape and the accuracy of the motion process.

% Some approaches are designed to be applied on specific dataset  or in dedicate scenario, e.g. \cite{Ruben2018Longterm}uses human pose information as additional supervision.
% \cite{guen2020disentangling} makes use of physical information by introducing partial differential equations(PDEs) to improve prediction performance. 
% While our model use only self-supervised learning without any prior acknowledge to reach state-of-the-art performances on Human3.6M. With a gain of 33 points, our performance gain is large on MSE metric while close on SSIM, LPIPS, and PSNR comparing to PhyDNet.
% The prediction result comparison is visualized in figure\ref{fig:human}. In the results of LMC-Memory, we found human's legs are severely deformed comparing to groundtruth. The human part of results of Motion-RNN and PhyDNet are obviously not as clear as ours.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/kitti.pdf}
	\caption{Prediction examples on KITTI dataset. 
	}
	\label{fig:KITTI}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/weather.pdf}
	\caption{Prediction examples on Weather dataset. 
	}
	\label{fig:weather}
\end{figure}



\subsection{IS MIMO beats SISO ?}
\label{sec:IS MIMO beats SISO ?}
Finally, we compare against the state-of-the-art over all four datasets. 

\noindent \textbf{Results on Moving MNIST.}
Firstly, we evaluate the performance of our MIMO-VP with the state-of-the-art methods on 10-10 task, which means 10 frames are used to predict 10 future frames. 
As shown in \Cref{Tab: Moving MNIST}, our model significantly outperforms all the other models.
%gains a huge performance improvement and achieves the best performance. 
In detail, compared with PhyDNet, our model improves $26.9\%$ and $26.6\%$in terms of MSE ans MAE respectively.  
As shown in \Cref{fig:mnist}, at the beginning, the two digits stick together and then gradually keep away from each other.
Current RNN-based models get blurry and wrong predictions in this case, and their prediction error largen over time.
On the contrary, our model can predict precise and clear frames. 

To further explore the performance of our MIMO-VP on long-term prediction, we conduct an experiment by predicting 30 future frames conditioned on 10 input frames. 
As shown in \Cref{Tab: Moving MNIST}, our method far surpasses the others in predicting 30 frames in terms of the MSE metric. 
Compared with PhyDNet, our MIMO-VP improves $46.2\%$ in MSE , which is much larger than $26.9\%$ in 10-10 prediction task. 
From the comparison, we can conclude that our MIMO-VP captures the long-term spatiotemporal dependency both in the input frames and output frames. 
Furthermore, our model has more advantages in predicting long-term sequences. 
%The visualization results of 10-30 task is shown in supplementary materials. 

\begin{table*}[h]
%\small
\centering
\tabcolsep3pt
\caption{Quantitative comparison of different models on KITTI dataset.}
  \begin{tabular}{l|cccc}
  \hline
    Method   & MAE/100 $\downarrow$ & SSIM $\uparrow$& LPIPS $\downarrow$ & PSNR $\uparrow$ \\
	\hline 
	\hline
	CrevNet \cite{yu2019crevnet} & 56.3 & 0.587  & 0.454  & 17.046  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 1005.3 & 4092.9 & 0.695\\
		PhyDNet \cite{guen2020disentangling}  & 44.9 & 0.674  & 0.403& 19.159 \\
		LMC-Memory \cite{lee2021video}  & 44.6 & 0.660  &  0.410  & 18.692\\
		MotionRNN \cite{wu2021motionrnn}  & 45.0 & 0.652  & 0.384& 18.931 \\
		\textbf{Predformer}  & \textbf{40.9} & \textbf{0.703} & \textbf{0.308}& \textbf{19.616}  \\
     \hline
	\end{tabular}
\label{Tab: kitti}
\end{table*}

\begin{table*}[h]
\centering
\caption{Quantitative comparison of different models on Weather dataset.}
\tabcolsep 8pt
  %\small
  \begin{tabular}{l|cccc}
  \hline
    Method  & MAE $\downarrow$ & SSIM $\uparrow$ & CSI-20 $\uparrow$ & CSI-30 $\uparrow$\\
	\hline 
	\hline
	MIM \cite{wang2019memory}  & 402.6 & 0.725& 0.402  & 0.164\\
		% 		CrevNet \cite{yu2019crevnet} & 962.4 & 0.786  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 51.0 & 223.0 & 0.847\\
		PhyDNet \cite{guen2020disentangling}  & 280.1 & 0.859 & 0.557 & 0.368 \\
		MotionRNN \cite{wu2021motionrnn}  & 336.9 & 0.809 & 0.519 & 0.290 \\
		\textbf{Predformer}  & \textbf{235.6} & \textbf{0.865} & \textbf{0.595} & \textbf{0.400}\\ 
     \hline
	\end{tabular}
\label{Tab: weather}
\end{table*}


\noindent \textbf{Results on Human3.6M.}
%Human action is one of the most difficult task in video prediction domain. 
%From Table \ref{Tab: human}, we can see that our proposed MIMO-VP achieves the best performance compared with other methods. 
%From Figure \ref{fig:human} we also can see that our model predicts comparable result with the state-of-the-art methods. 
%However, we have to say the performance of all these models are not as perfect as we expect. 
%Thesefore, how to model the non-rigid active of human body is a much challenging task, which is left for future work.
\Cref{Tab: human} shows that MIMO-VP achieves the best performance on Human3.6M. 
Compared with PhyDNet, MIMO-VP improves $35.8\%$ in MAE. 
%In \Cref{fig:human}, the background is complicated and gives much more challenge for modeling. 
%From the visualization results , we can see that our model still can product reasonable results while other models get quite blurry predictions.
In \Cref{fig:human}, complicated background and human motion give much more challenge for predicting accurate and reasonable results. While our MIMO-VP can still product relatively precise future frames comparing with other models.
%Some approaches e.g.\cite{Ruben2018Longterm} uses human pose information as additional supervision.

% From Figure \ref{fig:human} we can see that in the result of LMC-Memory, obvious deformation appears on human legs. 
% In the result of MotionRNN and PhyDNet, the upper human body is unreasonably slim and obese comparing to groundtruth.
% While our model MIMO-VP can take into account the rationality of the overall human shape and the accuracy of the motion process.

% Some approaches are designed to be applied on specific dataset  or in dedicate scenario, e.g. \cite{Ruben2018Longterm}uses human pose information as additional supervision.
% \cite{guen2020disentangling} makes use of physical information by introducing partial differential equations(PDEs) to improve prediction performance. 
% While our model use only self-supervised learning without any prior acknowledge to reach state-of-the-art performances on Human3.6M. With a gain of 33 points, our performance gain is large on MSE metric while close on SSIM, LPIPS, and PSNR comparing to PhyDNet.
% The prediction result comparison is visualized in figure\ref{fig:human}. In the results of LMC-Memory, we found human's legs are severely deformed comparing to groundtruth. The human part of results of Motion-RNN and PhyDNet are obviously not as clear as ours.





\noindent \textbf{Results on KITTI.}
%Kitti is a complex real dataset with varying camera positions and scenes, which give much challenge to model the variation of both scenes and moving objects. 
As shown in \Cref{Tab: kitti}, our proposed MIMO-VP achieves consistent improvement in all evaluation metrics. 
Compared with LMC-Memory, our model improves $8.3\%$ in MAE.
Quantitative visualization results in \Cref{fig:KITTI} show that our model can preserve much more details of both background and foreground. 
For instance, from the right part of last predicted frames, we can find that the results of our MIMO-VP is much similar to GroundTruth while other methods produce obviously blurry frames. 

\noindent \textbf{Results on Weather.}
%Precipitation nowcasting is a significant application of video prediction, which is much meaningful for human dail life. 
%We collect and process the raw data from local weather bureau and make this dataset for verifying the performance of our MIMO-VP on precipitation nowcasting task. 
From Table \ref{Tab: weather}, we can find that our MIMO-VP has significantly improvement in CSI scores with different thresholds, which indicates our approach can predict more credible radar echoes for precipitation nowcasting. 
%The CSI score is commonly used in  precipitation nowcasting domain. 
The visualization radar echo maps are shown in \Cref{fig:weather}. Different color represents different radar echo intensity (dBZs), \ie \ yellow indicates higher intensity than green.
Additionally, the center region of the radar echo is zoomed in and placed below each predicted frame. 
We find that our MIMO-VP predicts more correct yellow regions  than other methods, which means MIMO-VP is a more suitable method for precipitation nowcasting.

% \noindent \textbf{Results on KITTI.}
% %Kitti is a complex real dataset with varying camera positions and scenes, which give much challenge to model the variation of both scenes and moving objects. 
% As shown in \Cref{Tab: kitti}, our proposed MIMO-VP achieves consistent improvement in all evaluation metrics. 
% Compared with LMC-Memory, our model improves $8.3\%$ in MAE.
% Quantitative visualization results in \Cref{fig:KITTI} show that our model can preserve much more details of both background and foreground. 
% For instance, from the right part of last predicted frames, we can find that the results of our MIMO-VP is much similar to GroundTruth while other methods produce obviously blurry frames. 

% \noindent \textbf{Results on Weather.}
% %Precipitation nowcasting is a significant application of video prediction, which is much meaningful for human dail life. 
% %We collect and process the raw data from local weather bureau and make this dataset for verifying the performance of our MIMO-VP on precipitation nowcasting task. 
% From Table \ref{Tab: weather}, we can find that our MIMO-VP has significantly improvement in CSI scores with different thresholds, which indicates our approach can predict more credible radar echoes for precipitation nowcasting. 
% %The CSI score is commonly used in  precipitation nowcasting domain. 
% The visualization radar echo maps are shown in \Cref{fig:weather}. Different color represents different radar echo intensity (dBZs), \ie \ yellow indicates higher intensity than green.
% Additionally, the center region of the radar echo is zoomed in and placed below each predicted frame. 
% We find that our MIMO-VP predicts more correct yellow regions  than other methods, which means MIMO-VP is a more suitable method for precipitation nowcasting.







==> PaperBody/experiment2.tex <==
\subsection{Dataset Descriptions}

\noindent \textbf{Moving MNIST} \cite{srivastava2015unsupervised} is a standard synthetic dataset for video prediction. We generate the training set following \cite{guen2020disentangling},
and adopt the widely used test set of 10,000 sequences provided by \cite{srivastava2015unsupervised}. 

\noindent \textbf{Human3.6M} \cite{ionescu2013human3} dataset is a real-world human pose dataset comprising 17 kinds of human actions and 3.6 million poses. We use subjects S1, S5, S6, S7 and S8 for training, and subjects S9, S11 for testing. We predict $4$ frames in the future conditioned on the $4$ observed frames.

\noindent \textbf{Weather} dataset is a real radar echo dataset for precipitation nowcasting, which is obtained from the local weather bureau. Our training set and testing set contain $9,600$ and $2400$ radar sequences (resolution 128$\times$128$\times$1) respectively.

\noindent \textbf{KITTI} dataset is one of the most popular datasets for autonomous driving and also a benchmark for computer vision algorithms. We predict $5$ frames in the future when takes $5$ observed frames as input.

\subsection{Implementation Details}
We use Adam \cite{kingma2014adam} with 0.0005 learning rate to train our model. ReduceLROnPlateau is adopted to reduce the learning rate with 0.5 decay factor when loss stop decreasing. For Moving MNIST dataset, we use 6 transformer blocks in the encoder and 10 blocks in the decoder. We implemented the model with PyTorch and conducted experiments on NVIDIA V100 GPUs. Mean Squared Error (MSE), Mean Absolute Error (MAE), the Structural Similarity(SSIM), LPIPS~\cite{zhang2018unreasonable} and Peak Signal to Noise Ratio (PSNR) are evaluated in our work. All these metrics are averaged for all predicted frames. Additionally, we also take Critical Success Index (CSI) into account for Weather dataset. More details are contained in \textit{supp}. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/mnist.pdf}
	\caption{Prediction examples on Moving MNIST dataset. 
	}
	\label{fig:mnist}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/human.pdf}
	\caption{Prediction examples on Human3.6M dataset. 
	}
	\label{fig:human}
\end{figure}


\begin{table}[t]
	%\small
	\centering
	\tabcolsep 9pt
	\caption{Quantitative comparisons on Human3.6M dataset.}
	\scalebox{0.9}{
	\begin{tabular}{l|ccc}
		\hline
		Method   & MAE/100 $\downarrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ \\
		\hline 
		\hline
		MIM & 17.8& 0.790 & 20.57  \\
		PhyDNet & 16.2 & 0.901 &-\\
		LMC-Memory  & 17.0 & 0.820 &21.05\\
		MotionRNN  & 14.8& 0.846 & 22.16   \\
		\textbf{MIMO-VP}  & \textbf{10.4} & \textbf{0.941}  & \textbf{24.52} \\
		\hline
	\end{tabular}}
	\label{Tab: human}
\end{table}

\begin{table}[t]
%\small
\centering
\tabcolsep3pt
\caption{Quantitative comparisons on KITTI dataset.}
  \begin{tabular}{l|cccc}
  \hline
    Method   & MAE/100 $\downarrow$ & SSIM $\uparrow$& LPIPS $\downarrow$ & PSNR $\uparrow$ \\
	\hline 
	\hline
	CrevNet & 56.3 & 0.587  & 0.454  & 17.046  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 1005.3 & 4092.9 & 0.695\\
		PhyDNet   & 44.9 & 0.674  & 0.403& 19.159 \\
		LMC-Memory  & 44.6 & 0.660  &  0.410  & 18.692\\
		MotionRNN  & 45.0 & 0.652  & 0.384& 18.931 \\
		\textbf{MIMO-VP}  & \textbf{40.9} & \textbf{0.703} & \textbf{0.308}& \textbf{19.616}  \\
     \hline
	\end{tabular}
\label{Tab: kitti}
\end{table}

\begin{table}[t]
\centering
\caption{Quantitative comparisons on Weather dataset.}
\tabcolsep 8pt
  %\small
  \scalebox{0.9}{
  \begin{tabular}{l|cccc}
  \hline
    Method  & MAE $\downarrow$ & SSIM $\uparrow$ & CSI-20 $\uparrow$ & CSI-30 $\uparrow$\\
	\hline 
	\hline
	MIM  & 402.6 & 0.725& 0.402  & 0.164\\
		% 		CrevNet \cite{yu2019crevnet} & 962.4 & 0.786  \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 51.0 & 223.0 & 0.847\\
		PhyDNet & 280.1 & 0.859 & 0.557 & 0.368 \\
		MotionRNN & 336.9 & 0.809 & 0.519 & 0.290 \\
		\textbf{MIMO-VP}  & \textbf{235.6} & \textbf{0.865} & \textbf{0.595} & \textbf{0.400}\\ 
     \hline
	\end{tabular}}
\label{Tab: weather}
\end{table}



\begin{table*}[t]
	%\small
	\centering
	\tabcolsep8pt
	\caption{Quantitative comparison of different methods on Moving MNIST and KITTI datasets. In the third column, "R" and "T" denotes RNN and Transformer architecture respectively.}
	\begin{tabular}{l|c|c|cc|cc}
		\hline
		\multicolumn{3}{c|}{}& \multicolumn{2}{c|}{Moving MNIST}  & \multicolumn{2}{c}{KITTI} \\
		\hline
		Method  & Type & Network &MSE $\downarrow$ & MAE $\downarrow$ & MAE/100 $\downarrow$ & SSIM $\uparrow$ \\
		\hline 
		\hline
		PhyDNet & SISO & R & 24.2 & 70.3 & 44.9 & 0.674 \\
		HORST & SISO & T & 26.5 & 75.5 & 53.3 & 0.571 \\
		MISO-VP & MISO & T &22.8 & 62.8 & 42.1 & 0.690 \\
		\textbf{MIMO-VP} & MIMO & T & \textbf{17.7} & \textbf{51.6} & \textbf{40.9}  & \textbf{0.703}  \\
		\hline
	\end{tabular}
	\label{Tab: mimo}
\end{table*}

\begin{table}[t]
%\small
\centering
\tabcolsep3pt
\caption{Results of MIMO models on Moving MNIST.}
  \begin{tabular}{l|ccccc}
  \hline
    Method   & MSE & MAE $\downarrow$ & SSIM $\uparrow$\\
	\hline 
	\hline
		MAU & 27.6 & 79.4 & 0.937   \\
	\hline	
	3D convolution  & 32.8 & 84.4 & -   \\
		%Conv-TT-LSTM \cite{su2020convolutional} & 1005.3 & 4092.9 & 0.695\\
		ViT \cite{dosovitskiy2020image}& 50.2 & 126.5 & 0.887  \\
		Swin-transformer \cite{liu2021swin}& 28.8 & 77.2 & 0.940  \\
		SimVP \cite{gao2022simvp} & 23.8& 68.9 & 0.948 \\
		\textbf{MIMO-VP} & \textbf{17.7}  & \textbf{51.6} & \textbf{0.964}   \\
     \hline
	\end{tabular}
\label{Tab: MIMO_compare}
\end{table}



\subsection{Overall performance compared with the state-of-the-art}
\label{sec:IS MIMO beats SISO ?}
\noindent \textbf{Results on Moving MNIST.}
Firstly, we report the comparison experiments which use 10 frames to predict 10 future frames. As shown in \Cref{Tab: Moving MNIST} and \Cref{fig:mnist}, our model significantly outperforms all the other models. Current RNN-based models get blurry and wrong predictions in this case, and their prediction error grows larger over time. On the contrary, our model can predict high quality frames. 

To further explore on long-term prediction, we conduct an experiment by predicting 30 future frames conditioned on 10 input frames. As shown in \Cref{Tab: Moving MNIST}, our method far surpasses the others in predicting 30 frames in terms of the MSE metric. Compared with PhyDNet, our MIMO-VP improves $46.2\%$ in MSE , which is much larger than $26.9\%$ in 10-10 prediction task. From the comparison, we can conclude that our MIMO-VP captures the long-term spatiotemporal dependency both in the input frames and output frames. 



\noindent \textbf{Results on Human3.6M.}
\Cref{Tab: human} shows that MIMO-VP win the rank 1 place on Human3.6M. 
Compared with PhyDNet, MIMO-VP improves $35.8\%$ in MAE. 
In \Cref{fig:human}, complicated background and human motion give much more challenge for predicting accurate and reasonable results. 

\noindent \textbf{Results on KITTI.}
As shown in \Cref{Tab: kitti}, our proposed MIMO-VP achieves consistent improvement in all evaluation metrics. Quantitative visualization results in supplemental materials show that our model can preserve much more details of both background and foreground. 

\noindent \textbf{Results on Weather.}
From Table \ref{Tab: weather}, we can find that our MIMO-VP has significantly improvement in CSI scores with different thresholds, which indicates our approach can predict more creditable radar echoes for precipitation nowcasting. 
The visualization radar echo maps are included in supplementary materials. We find that our MIMO-VP predicts more correct heavily raining regions than other methods, which means MIMO-VP is a more suitable method for precipitation nowcasting.

\subsubsection{\textbf{The comparison of different MIMOs}}
The comparison of different MIMO methods and the best SISO method is shown in Table~\ref{Tab: MIMO_compare}. We first observe that all other MIMO methods can not achieve state-of-the-art performance when compared with the best SISO method--MAU \cite{chang2021mau} except ours. 

\begin{table}[t]
	%\small
	\centering
	\tabcolsep0.8pt
	\caption{Ablation Study for Each Components.}
	\begin{tabular}{l|cc|cc}
		\hline
		& \multicolumn{2}{c|}{Moving MNIST}  & \multicolumn{2}{c}{KITTI} \\
		\hline
		Method  & MSE $\downarrow$ & MAE $\downarrow$ & MAE/100 $\downarrow$ & SSIM $\uparrow$ \\
		\hline  
		\hline
		Independent & 21.6 & 59.4 & 41.5 & 0.695 \\
		Without 2DMHA & 32.8 & 84.4 & 44.6 & 0.663 \\
		Without LSB  & 21.2 & 59.2 & 42.3 & 0.687 \\
		%MIMO-VP w/ Recurrent & 22.8 & 62.8 & 42.1 & 0.690 \\
		\hline
		\textbf{MIMO-VP}  & \textbf{17.7} & \textbf{51.6} & \textbf{40.9}  & \textbf{0.703}  \\
		\hline
	\end{tabular}
	\label{Tab: ablation}
\end{table}




\subsection{Ablation Study of Each Component in MIMO-VP}
\label{sec:Which MIMO?}
We carry out an ablation study to analyse the respective contributions of the operations which we proposed for MIMO-VP. Quantitative results on Moving MNIST and KITTI datasets are shown in \Cref{Tab: ablation}. (1) \textbf{The Spatial Dependency of Frames}. Without MHA, the model drops  $15.1$ and $32.8$ in terms of MSE and MAE respectively on the Moving MNIST. (2) \textbf{The Local Spatio-temporal Block}. This block introduces XXX maximal perfromance gains on XXX dataset. (3) \textbf{The Multi-Out Decoder}. We design a baseline MISO-VP which adopts Transformer architecture but infers the next one frame using the last predicted frame in a recursive manner. Experimental results are shown in \Cref{Tab: mimo}. On the Moving mnist dataset by predicting 10 future frames, MIMO-VP beats down the MISO-VP with performance improves by $18.0\%$ and $14.0\%$ in MSE and MAE respectively. The reason may be that recursive single-out predictive strategy will trigger the error accumulation problem and overlook the stochastic dependency among the future frames.

\begin{figure}[t]
	\centering
	\begin{subfigure}[]{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/long-term.pdf}
		\caption{MSE w.r.t input length}
		\label{figure:long-term}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/error.pdf}
		\caption{Frame-wise MSE}
		\label{figure:error accumulation}
	\end{subfigure}
	\caption{Comparison of MIMO-VP and PhyDNet by predicting 10 future frames.}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{subfigure}[]{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/longterm-mae.pdf}
		\caption{MAE w.r.t Output length}
		\label{figure:long term prediction1}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/longterm-ssim.pdf}
		\caption{SSIM w.r.t Output length}
		\label{figure:long term prediction2}
	\end{subfigure}
	\caption{The mean MAE (a) and SSIM (b) by using 10 frames to  predict 10, 30, 50 and 90 frames.}
\end{figure}





\subsection{Comparison of MIMO and SISO}
\label{sec:Why MIMO beats SISO?}
\subsubsection{\textbf{Analysis of the Error Accumulation}}
\Cref{figure:error accumulation} illustrates the frame-wise MSE results of MIMO-VP and PhyDNet, corresponding to the sample in \Cref{fig:mnist}, and lower curves denote higher prediction accuracy. We observe that the frame wise MSE of PhyDNet is increase obviously when compared with our MIMO-VP.
These comparison results prove that with the help of MIMO strategy, MIMO-VP can overcome the error accumulation.

\subsubsection{\textbf{Significance of `MI'}}
To investigate how the MIMO-VP is capable of capturing the long-term relationships of sequence,
we conduct experiment on Moving mnist dataset by predicting 10 future frames conditioned on $50$ observed frames.
Comparison results between MIMO-VP and PhyDNet of predicting 10 future frames on Moving MNIST with different input lengths are shown in \Cref{figure:long-term}.
Those results demonstrate that our MIMO-VP has a stronger ability to capture the long-term sptiotemporal dependency of video sequences for accurate prediction,
while PhyDNet, an RNN-based method, suffers from the long-term dependency problem because of the limited capacity of memory.

\subsubsection{\textbf{Significance of `MO'}} To verify the effectiveness of the MIMO strategy on long-term prediction, we compare the results of predicting 10,30,50 and 90 frames on Moving MNIST dataset. 
In training phase, all the models are trained by using 10 frames to predict next 10 frames, while in testing phase, 10, 30, 50, and 90 frames are predicted in a recurrent manner. 
Experimental results are shown in Figure XXX, from which we can observe that our model achieve the state-of-the-art performance on all 4 long-term time scales. 


\subsubsection{\textbf{Speed and accuracy trade-off}}
From \Cref{Tab: Inference Time}, we can observe that our `MO' methods runs much faster than `SO' methods. According to \Cref{figure:long term prediction1}, \Cref{figure:long term prediction2}, we can see that MIMO-VP can achieve state-of-the-art performance with a comparable inference time, which can serve as a backbone for future research. 

\begin{table}[h]
%\small
\centering
\tabcolsep3pt
\caption{Inference time on Moving MNIST.}
  \begin{tabular}{l|ccccc}
  \hline
    Models   & PhyDNet & SimVP  & MotionRNN & MIMO-VP\\
	\hline 

	10-30 & 0.2274s & 0.0643s & 0.6299s & 0.1498s    \\

     \hline
	\end{tabular}
\label{Tab: Inference Time}
\end{table}


















==> PaperBody/limitation.tex <==
The proposed Predormer encodes the whole input sequences at once, which needs significantly large GPU memory.  Furthemore, the self-attention operation is quadratically increase with input length, which can be optimize in future works . Lastly, the MIMO strategy is not flexible, which can not be used to predict future frames with variational output length.

==> PaperBody/proposedmethod.tex <==

\subsection{Spatiotemporal Sequence Prediction}

Suppose we observe a video sequence $\ \mathcal{S}_{t-m+1:t} := \{\mathcal{X}_{t-m+1},$ $\mathcal{X}_{t-m+2}, \dots, \mathcal{X}_t \}$, 
where $\mathcal{X}_t\in \mathbb{R}^{C_0\times H_0\times W_0}$ represents the frame (channel $C_0$, height $H_0$, width $W_0$) at the current timestep $t$.
The goal of the spatiotemporal sequence prediction is to generate the most likely length-$n$ sequence in the future given the previous length-$m$ sequence including the current observation:
\begin{equation}
\begin{split}
\mathcal{S}^*_{t+1:t+n} = \mathop{\arg\max}\limits_{\mathcal{S}_{t+1:t+n}} \  p(\mathcal{S}_{t+1:t+m} | \mathcal{S}_{t-m+1:t})
\end{split}
\label{eq: Spatiotemporal Sequence Prediction}
\end{equation}
\noindent \textbf{SISO predictive strategy.} 
To solve the above problem, RNN-based models usually adopt the SISO strategy that outputs a single next frame taking as input the current frame.
The SISO prediction paradigm can be expressed as:
\begin{equation}
\begin{split}
\mathcal{X}_{t'+1} = F(\mathcal{X}_{t'}, M_{t'})+\sigma_{t'},
\end{split}
\label{eq: RNN_solve}
\end{equation}
where $F$ denotes the model, $M_{t'}$ is the memory cell that remembers the past historical information.
$\sigma_{t'}$ is a Tensor noise term.
$\mathcal{X}_{t'}$ is the observed frame ($t'\leq t$) or the generated frame ($t'>t$).
%After repeating $n+m-1$ times, the sequence $\mathcal{S}_{t+1:t+m}$ that contains the last $n$ frames is the final result.
Note that SISO predictive strategy is susceptible to the error accumulation problem.
For simplicity, consider an AutoRegressive with $K$=$1$ and without exogenous inputs model:
\begin{equation}
\begin{split}
\mathcal{X}_{t} = A\mathcal{X}_{t-1}+\sigma_{t}
\end{split}
\label{eq: AutoRegressive}
\end{equation}
where $A$ is a learnable Tensor. 
It is easy to have:
\begin{equation}
\begin{split}
\mathcal{X}_{t+n} = A^{t+n-1}\mathcal{X}_{t}+\sum_{k=t}^{t+n-1}A^k\sigma_{t+n-k}+\sigma_{t+n}
\end{split}
\label{eq: error}
\end{equation}
It is clear that the error $R_{t+n}=\sum_{k=t}^{t+n-1}A^k\sigma_{t+n-k}+\sigma_{t+n}$ will accumulate as timestep $t+n$ increases,
which makes accurate prediction challenging.
Besides, the long-term dependency problem inherited from RNNs would further limit the performance of the SISO strategy on video prediction.

\noindent \textbf{MIMO predictive strategy.} 
We propose in this paper a novel multiple-in-multiple-out predictive strategy:
\begin{equation}
\begin{split}
\mathcal{S}_{t+1:t+n} = F(\mathcal{S}_{t-m+1:t})+ \Sigma_{t+1:t+n},
\end{split}
\label{eq: our_solve}
\end{equation}
where $\Sigma_{t+1:t+n}:=\{\sigma_{t+1},\dots,\sigma_{t+n}\}$ is the normal prediction error.
Two attractive properties of this MIMO strategy are:
(1) it is free of error accumulation without the recurrent structure, which facilitates accurate prediction by taking as input the confident observed sequence;
(2) it generates the whole sequence $\mathcal{S}_{t+1:t+n}$ in parallel, which improves  accuracy by preserving the dependency between futures.
However, it is non-trivial to apply this strategy for video prediction because it demands the ability to model long-term spatiotemporal dependencies of sequence.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/model.pdf}
	\caption{\textbf{Illustration of Predormer architecture.} It contrains two main components: 1) a 2D convolutional multi-head attention (2DMHA); and 2) a 3D convolutional feed-forward networks (3DFFN). Predormer predicts target video sequences in parallel.
	}
	\label{fig:model}
\end{figure}
\subsection{Predormer Architecture}
We introduce a MIMO video prediction model built upon Transformer \cite{vaswani2017attention}, termed as Predormer, which is an encoder-decoder architecture, as depicted in \Cref{fig:model}.
The building block for Predormer mainly consists of two modules:
a 2D convolutional Multi-Head Attention (2DMHA) that helps to capture the global long-term motion trend of sequence,
and a 3D convolutional Feed-Forward Network (3DFFN) that focuses on modeling the local short-term variation of sequence. 
The overall learning procedure of Predormer is expressed as:
\begin{equation}
\mathcal{S}_{t+1:t+n} = \Phi_d(\Phi_e(\mathcal{S}_{t-m+1:t}), \mathcal{T}_{t+1:t+n})
\label{eq: learning procedure}
\end{equation}
where $\Phi_e$ and $\Phi_d$ are the encoder and decoder modules respectively. $\mathcal{T}_{t+1:t+n}$ is a length-$n$ timestep queries. For an input video $\mathcal{S}_{t-m+1:t}\in \mathbb{R}^{m\times C_0\times H_0 \times W_0}$ with $m$ frames, we first decompose each frame into non-overlapping patches and then obtain the sequence-level feature maps $h\in \mathbb{R}^{m\times C \times H\times W}$ after several convolution layers. Details of the subsequent 2DMHA and 3DFFN are as follow.
% \noindent \textbf{Feature embedding.}
% For an input video sequence $\mathcal{S}_S\in \mathbb{R}^{S\times C_0\times H_0 \times W_0}$ with $S$ frames,
% we first decompose each frame into non-overlapping patches by a patch splitting module to downscale their resolution.
% Then a $3\times 3$ convolution, followed by a GroupNorm and the SiLU activation function, is applied on each frame to obtain a feature map with an arbitrary channel $C$,
% resulting in the final sequence-level feature map $h\in \mathcal{R}^{S\times C \times H\times W}$.

\noindent \textbf{2DMHA.}
The core issue for pixel-level video prediction is long-term spatiotemporal sequence modeling.
While the vanilla Transformer \cite{vaswani2017attention} has proven powerful for modeling long-range relationships of sequence in machine translation,
it is also important to preserve the spatial information of frames for video prediction.
To compensate for this limitation, we propose to incorporate the convolutional structures into the multi-head attention to simultaneously model the temporal correlation and preserve the spatial information of sequence. 
Given a sequence-level feature map $h\in \mathbb{R}^{m\times C \times H\times W}$ (similarly, $h'\in \mathbb{R}^{n\times C \times H\times W}$ in the decoder),
we apply 2D convolutions to generate the query map and paired key-value
map of each frame:
\begin{equation}
	Q, K, V \in \mathbb{R}^{m\times C \times H\times W} = \Theta_{q}(h), \Theta_{k}(h), \Theta_{v}(h)
\end{equation}
where $\Theta_{q}$, $\Theta_{k}$ and $\Theta_{v}$ are $1\times 1$ convolutions.
Then we compute the output feature maps by Scaled Dot-Product Attention as:
\begin{equation}
\textup{Attention}(Q,K,V)=\textup{SoftMax}(\frac{QK^T}{\sqrt{d_k}})V
\end{equation}
where $d_k=C*H*W$, $QK^T\in \mathbb{R}^{m\times m}$ is the temporal attention map of the input sequence.
Finally, the 2DMHA with $h$ heads used in our work can be expressed as:
\begin{equation}
\begin{split}
\textup{2DMHA}(Q,K,V)=\Theta_o(\textup{Concat}(\textup{head}_1,\dots,\textup{head}_h))\\
\textup{where head}_i = \textup{Attention}(\Theta_{q_i}(h), \Theta_{k_i}(h), \Theta_{v_i}(h))
\end{split}
\end{equation}
where $\Theta_{q_i}$, $\Theta_{k_i}$ and $\Theta_{v_i}$ are $1\times 1$ convolutions with output channel of $C/h$.

Note that, in each decoder block, different from the existing auto-regressive prediction paradigm of Transformers,
we do not apply the mask operation on the multi-head self-attention,
because our decoder inputs are timestep encodings that are already known.
In such a manner, 
the decoder can generate efficiently multiple future frames within one-step forward inference, so as to avoid error accumulation.
In addition,
each generated frame is conditioned not only on the past sequence but also on its future frames,
which makes Predormer capable of preserving the dependency of future frames.

\noindent \textbf{3DFFN.}
While 2DMHA can model the long-term motion trend of sequences, we find that the short-term variation of sequences is also crucial for video generation.
We, therefore, propose to adopt the 3D convolutions to model the local spatiotemporal relations among frames,
so as to learn the high order relationship between timestep queries $\mathcal{T}$ and their corresponding output sequence $\mathcal{S}$.
The 3DFFN used in our Predormer architecture consists of two embedding layers with each is a \texttt{3DConv}, \texttt{LayerNorm}, \texttt{SiLU} block.
The kernel size of \texttt{3DConv} is $3\times 3\times 3$.

\begin{comment}
Given a feature map $\mathcal{Z}$ output from 2DMHA, the computing of the 3DFFN is:
\begin{equation}
\begin{split}
\hat{\mathcal{Z}} &= \text{SiLU}(\textup{LayerNorm}(\Theta_{z_1}(\mathcal{Z})))\\
\bar{\mathcal{Z}} &= \textup{SiLU}(\textup{LayerNorm}(\Theta_{z_2}(\hat{\mathcal{Z}})))\\
\textup{3DFFN}(\mathcal{Z}) &= \textup{LayerNorm}(\mathcal{Z}+\bar{\mathcal{Z}})
\end{split}
\end{equation}
where $\Theta_{z_1}$ and $\Theta_{z_2}$ are $3\times 3\times 3$ convolutions with output channel of $C$.
\end{comment}

\noindent \textbf{Temporal positional encoding and timestep quires.}
Considering the permutation-invariant character of the Transformer architecture,
%it is important to maintain the order information of the video sequence.
we here focus on the temporal positional encoding of the sequence because the convolutional operation is adopted to preserve the structure information of frames.
We define a timestep vector $T=[1,2,\dots,m+n]$.
Then we embed $T\in \mathbb{R}^{1\times (m+n)}$ to $\hat{T}\in \mathbb{R}^{(m+n)\times C}$ by an embedding layer.
Finally, we expanse $\hat{T}$ to $\mathcal{T}\in \mathbb{R}^{(m+n)\times C\times H\times W}$ along the height and width dimensions.
Accordingly, the temporal positional encoding of input sequence is $\mathcal{T}_{1:m} \in \mathbb{R}^{m\times C\times H\times W}$.
And we regard $\mathcal{T}_{m+1:m+n}\in \mathbb{R}^{n\times C\times H\times W}$ as timestep queries and input them to the decoder module.

\subsection{Learning Objectives.}
We adopt two widely used content losses, \ie, \textbf{MSE loss} and \textbf{MAE loss}, after each decoder layer to guide the model training.
The loss function $\mathcal{L}$ can be expressed as:
\begin{equation}
\mathcal{L} =  \|\mathcal{S}^*-\mathcal{S}\|_F^2+\|\mathcal{S}^*-\mathcal{S}\|_1,
\end{equation}
where $\mathcal{S}^*$ is the generated frame sequence and $\mathcal{S}$ is the corresponding GroundTruth.

==> PaperBody/relatedwork.tex <==
\textbf{Video prediction.}
Mainstream video prediction models \cite{xingjian2015convolutional,shi2017deep,wang2017predrnn,wang2018predrnn++,oliu2018folded,wang2018eidetic,wang2019memory,guen2020disentangling,Yu2020EfficientAI,lin2020self,su2020convolutional,wu2021motionrnn,lee2021video} are Recurrent Neural Networks (RNNs), which adopt the Single-In-Single-Out predictive strategy.
As a prior work,
Shi \emph{et al.} \cite{xingjian2015convolutional} incorporated convolutional operation into the LSTM framework (ConvLSTM) to perform spatiotemporal predictive learning for video forecasting problems.
After that, variants of ConvLSTM have been proposed.
PredRNN \cite{wang2017predrnn} proposed a novel spatiotemporal LSTM block to memory both spatial and temporal representations.
Wang \emph{et al.} \cite{wang2019memory} proposed the Memory in Memory networks (MIM) to model the high-order non-stationary variations of video sequences.
MotionRNN \cite{wu2021motionrnn} introduced the MotionGRU to decompose the video sequence into transient variation and motion trend.
Beyond the local spatial dependencies captured by convolution layers,
Lin \emph{et al.} \cite{lin2020self} integrated the self-attention mechanism into ConvLSTM (SA-ConvLSTM) to extract the long-range spatial dependencies of video frames.
Su \emph{et al.} \cite{su2020convolutional} proposed a higher-order convolutional recurrent network by the convolutional tensor-train decomposition.
In addition, disentangled representation learning also plays important role in video prediction.
MCnet\cite{villegas2017decomposing} and DRNET \cite{denton2017unsupervised} proposed to explicitly decompose each sequence frame into varying dynamics and a stationary content. 
PhyDNet \cite{guen2020disentangling} presented a two-branch deep architecture that disentangles physical dynamics into known dynamics and unknown factors based on the partial differential equations (PDEs).
Despite their promising performance,
previous SISO predictive models may suffer from the intractable error accumulation and long-term dependency problems,
which limits their further performance improvement in video prediction.
To alleviate the pixel-level error propagation in the long-term future, a lot of effort has been made.
Villegas \emph{et al.} \cite{villegas2017learning} propose to predict the human pose keypoints of the frames firstly and transfer them back into pixel space.
Another work in \cite{villegas2018hierarchical} resorts to predict a high-level encoding into the future, rather than the specific pose keypoints in \cite{villegas2017learning}.
Also, Lee \emph{et al.} \cite{lee2021revisiting} attempt to predict future frames by first estimating the semantic structures of video frames and subsequently translating the structures to pixels space.
These methods enhance their ability for long-term prediction by maintaining the consistency of the high-level structure of video sequences in the future.
In addition,
LMC-Memory\cite{lee2021video} propose to predict long term future frames by storing and recalling longterm motion contexts of video sequence.
Although achieving good results,
these methods can alleviate but not overcome the error accumulation problem inherited from the SISO predictive strategy.
%%Three MIMO methods. Mainly rely on 3D convolution
%Liu \emph{et al.} \cite{liu2017video} proposed DVF, which uses a 3D convolution autoencoder to learn voxel flows and synthesize video frames by flowing pixel values from existing ones.
%FutureGAN \cite{aigner2018futuregan} is also a encoder-decoder GAN model by stacking spatio-temporal 3d convolutions, it could predict multiple future frames at once.
%SimVP \cite{gao2022simvp} is a simple model that is completely built upon CNN. The MIMO predictive strategy of SimVP makes it outperforms existing SISO methods.
%However, the aforementioned approaches usually focus on modeling the short-term temporal motion while ignore the long-term motion trend of video sequences.
In this paper, we show that a novel Multiple-In-Multiple-Out predictive strategy can naturally and efficiently overcome the notorious error accumulation in long-term video prediction.

\textbf{Time Series Prediction.}
Over decades, time series prediction has been extensively studied in the literature.
It has been proved that the multiple-input multiple-output
(MIMO) approaches \cite{bontempi2008long,taieb2010multiple,taieb2009long} for multi-step-ahead time series prediction show superiority over the iterated single-output approaches and the direct single-output approaches.
The MIMO strategy breaks the error propagation chain in the iterated approach, and removes the conditional independence assumption which is implicit in the direct approach.
Inspired by this,
we propose a MIMO video prediction approach to improve the performance of the SISO strategy of existing RNNs.
However, compared to time series prediction,
video prediction is much more challenge due to the extremely complicate dynamics and visual representations of video sequences.

%Thanks to the success of the CNN and Transformers, we design a MIMO video prediction model built upon the convolutional Transformers.

==> PaperBody/relatedwork2.tex <==
\subsection{Single-In-Single-Out models}
Mainstream video prediction models \cite{xingjian2015convolutional,shi2017deep,wang2017predrnn,wang2018predrnn++,oliu2018folded,wang2018eidetic,wang2019memory,guen2020disentangling,Yu2020EfficientAI,lin2020self,su2020convolutional,wu2021motionrnn,lee2021video} follow the typical recurrent strategy to synthesis the future frames, which takes single frame in the sequence as input and output the next one by the recurrent unit.
As a prior work, Shi \emph{et al.}~\cite{xingjian2015convolutional} incorporated convolutional operation into the LSTM framework (ConvLSTM) to perform spatiotemporal predictive learning for video forecasting problems.
After that, variants of ConvLSTM have been proposed.
PredRNN \cite{wang2017predrnn} proposed a novel spatiotemporal LSTM block to memory both spatial and temporal representations.
Wang \emph{et al.} \cite{wang2019memory} proposed the Memory in Memory networks (MIM) to model the high-order non-stationary variations of video sequences.
MotionRNN \cite{wu2021motionrnn} introduced the MotionGRU to decompose the video sequence into transient variation and motion trend.
Beyond the local spatial dependencies captured by convolution layers, Lin \emph{et al.} \cite{lin2020self} integrated the self-attention mechanism into ConvLSTM (SA-ConvLSTM) to extract the long-range spatial dependencies of video frames.
Su \emph{et al.} \cite{su2020convolutional} proposed a higher-order convolutional recurrent network by the convolutional tensor-train decomposition.
In addition, disentangled representation learning also plays important role in video prediction.
MCnet\cite{villegas2017decomposing} and DRNET \cite{denton2017unsupervised} proposed to explicitly decompose each sequence frame into varying dynamics and a stationary content. 
PhyDNet \cite{guen2020disentangling} presented a two-branch deep architecture that disentangles physical dynamics into known dynamics and unknown factors based on the partial differential equations (PDEs).
However, it is still an inherent problem for all the aforementioned recurrent neural networks to capture long-term dependency and extrapolate longer sequence. 
To alleviate the pixel-level error propagation in the long-term future, a lot of effort has been made.
Villegas \emph{et al.} \cite{villegas2017learning} propose to predict the human pose keypoints of the frames firstly and transfer them back into pixel space.
Another work in \cite{villegas2018hierarchical} resorts to predict a high-level encoding into the future, rather than the specific pose keypoints in \cite{villegas2017learning}.
Also, Lee \emph{et al.} \cite{lee2021revisiting} attempt to predict future frames by first estimating the semantic structures of video frames and subsequently translating the structures to pixels space.
In addition, LMC-Memory\cite{lee2021video} propose to predict long term future frames by storing and recalling long-term motion contexts of video sequence.
Although these methods have achieved promising results by by maintaining the consistency of the high-level structure of videos, their error still accumulates in a compound rate according to the length of prediction.
In contrast, our model is build up on Multiple-In-Multiple-Out predictive strategy which fundamentally change the error propagation way rather than alleviating the error per frame.  

\subsection{Multiple-In-Multiple-Out models}
Instead of recurrent way, MIMO models generates all the future frames at once. It has been proved that these models \cite{bontempi2008long,taieb2010multiple,taieb2009long} for multi-step-ahead time series prediction show superiority over the others. However, MIMO models are lack of explore in video prediction field since this way may lose the time consistency of video data and generate noncontinuous motions since the temporal logic of the output frame is missing. Few attempts proposed MIMO-based models to anticipate videos but fails to beat the state-of-the-art SISO methods. For example, 
Liu \emph{et al.}~\cite{liu2017video} proposed DVF, which uses a 3D convolution autoencoder to learn voxel flows and synthesize video frames by flowing pixel values from existing ones. FutureGAN~\cite{aigner2018futuregan} is also a encoder-decoder GAN model by stacking spatio-temporal 3d convolutions, it could predict multiple future frames at once. SimVP~\cite{gao2022simvp} is a simple model that is completely built upon CNN. The MIMO predictive strategy of SimVP makes it achieving significant performance only with basic CNNs. However, we claim the real strength of MIMO architectures are still largely ignored and under exploited since they still fails to beats down some SISO models~\cite{XXX}. Thus we aim to develop a top-performing MIMO model to rise the attention for them in video prediction. 

\subsection{Transformer Models for Videos}
The advantage of modeling long-term dependency of video sequence enables Transformers~\cite{vaswani2017attention,dosovitskiy2020image,liu2021swin} to be widely applied in the video domain \cite{zhou2018end,gabeur2020multi,girdhar2019video,liu2020convtransformer,arnab2021vivit,dzabraev2021mdmmt,liu2021video,wang2021end,zhang2021token}.
For example, Zhou \emph{et al.} \cite{zhou2018end} proposed an end-to-end video captioning model based on transformer.
Kim \emph{et al.} \cite{kim2018spatio} proposed a novel Spatio-temporal Transformer Network (STTN) for Video Restoration. The works in~\cite{gabeur2020multi,dzabraev2021mdmmt} investigated the potential of Transformer on video retrieval tasks.
Besides, recent advances~\cite{girdhar2019video,zhang2021token,arnab2021vivit,liu2021video} focused on designing the transformer architectures for video classification.
VisTR~\cite{wang2021end} is a video instance segmentation framework based on an encoder-decoder Transformer structure,
which outputs the masks for each instance in the video in parallel.
However, the transformer architecture aiming at long-term video prediction is still underdeveloped and our work fills this gap. Experiments show that our non-trivial design leverages the performance of vanilla Transformer with a big margin. 


==> PaperBody/relatedwork3.tex <==
\noindent\textbf{Single-In-Single-Out models.}
Mainstream video prediction models \cite{xingjian2015convolutional,shi2017deep,wang2017predrnn,wang2018predrnn++,oliu2018folded,wang2018eidetic,wang2019memory,guen2020disentangling,Yu2020EfficientAI,lin2020self,su2020convolutional,wu2021motionrnn,lee2021video} follow the typical recurrent strategy to synthesis the future frames, which takes single frame in the sequence as input and output the next one by the recurrent unit.
As a prior work, Shi \emph{et al.}~\cite{xingjian2015convolutional} incorporated convolutional operation into the LSTM framework (ConvLSTM) to perform spatiotemporal predictive learning for video forecasting problems.
After that, variants of ConvLSTM have been proposed.
PredRNN \cite{wang2017predrnn} proposed a novel spatiotemporal LSTM block to memory both spatial and temporal representations.
Wang \emph{et al.} \cite{wang2019memory} proposed the Memory in Memory networks (MIM) to model the high-order non-stationary variations of video sequences.
MotionRNN \cite{wu2021motionrnn} introduced the MotionGRU to decompose the video sequence into transient variation and motion trend. 
PhyDNet \cite{guen2020disentangling} presented a two-branch deep architecture that disentangles physical dynamics into known dynamics and unknown factors based on the partial differential equations (PDEs).
However, it is still an inherent problem for them to capture long-term dependency and extrapolate longer sequence. 
To alleviate the pixel-level error propagation in the long-term future, a lot of effort has been made. Villegas \emph{et al.} \cite{villegas2017learning} propose to predict the human pose keypoints of the frames firstly and Lee \emph{et al.} \cite{lee2021revisiting} attempt to predict future frames by first estimating the semantic structures of video frames and subsequently translating the structures to pixels space. In addition, LMC-Memory\cite{lee2021video} propose to predict long term future frames by storing and recalling long-term motion contexts of video sequence.
However, all of their error still accumulates in a compound rate according to the length of prediction.
In contrast, our model is build up on MIMO predictive strategy which fundamentally change the error propagation way rather than alleviating the error per frame.  

\noindent \textbf{Multiple-In-Multiple-Out models.}
Instead of recurrent way, MIMO models generates all the future frames at once. It has been proved that these models \cite{bontempi2008long,taieb2010multiple,taieb2009long} for multi-step-ahead time series prediction show superiority over the others. However, MIMO models are lack of attention in video prediction field since this way may lose the time consistency of video data and generate noncontinuous motions since the temporal logic of the output frame is missing. Few attempts proposed MIMO-based models to anticipate videos but fails to beat the state-of-the-art SISO methods. For example, 
Liu \emph{et al.}~\cite{liu2017video} proposed DVF, which uses a 3D convolution autoencoder to learn voxel flows and synthesize video frames by flowing pixel values from existing ones. FutureGAN~\cite{aigner2018futuregan} is also a encoder-decoder GAN model by stacking spatio-temporal 3d convolutions, it could predict multiple future frames at once. SimVP~\cite{gao2022simvp} is a simple model that is completely built upon CNN. The MIMO predictive strategy of SimVP makes it achieving significant performance only with basic CNNs. However, we claim the real strength of MIMO architectures are still largely ignored and under exploited since they still fails to beats down top SISO models~\cite{chang2021mau}. Thus we aim to develop a top-performing MIMO model to rise the attention for them in video prediction. 

\noindent \textbf{Transformer Models for Videos}
The advantage of modeling long-term dependency of video sequence enables Transformers~\cite{vaswani2017attention,dosovitskiy2020image,liu2021swin} to be widely applied in the video domain \cite{zhou2018end,gabeur2020multi,girdhar2019video,liu2020convtransformer,arnab2021vivit,dzabraev2021mdmmt,liu2021video,wang2021end,zhang2021token}.
For example, Zhou \emph{et al.} \cite{zhou2018end} proposed an end-to-end video captioning model based on transformer.
Kim \emph{et al.} \cite{kim2018spatio} proposed a novel Spatio-temporal Transformer Network (STTN) for Video Restoration. The works in~\cite{gabeur2020multi,dzabraev2021mdmmt} investigated the potential of Transformer on video retrieval tasks.
Besides, recent advances~\cite{girdhar2019video,zhang2021token,arnab2021vivit,liu2021video} focused on designing the transformer architectures for video classification.
VisTR~\cite{wang2021end} is a video instance segmentation framework based on an encoder-decoder Transformer structure,
which outputs the masks for each instance in the video in parallel.
However, the transformer architecture aiming at long-term video prediction is still under developed and our work fills this gap. Experiments show that our non-trivial design leverages the performance of vanilla Transformer with a big margin. 

